Efficiently Learning Small Policies for Locomotion and Manipulation

Neural control of memory-constrained, agile robots requires small, yet highly performant models. We leverage graph hyper networks to learn graph hyper policies trained with off-policy reinforcement learning resulting in networks that are two orders of magnitude smaller than commonly used networks yet encode policies comparable to those encoded by much larger networks trained on the same task. We show that our method can be appended to any off-policy reinforcement learning algorithm, without any change in hyperparameters, by showing results across locomotion and manipulation tasks. Further, we obtain an array of working policies, with differing numbers of parameters, allowing us to pick an optimal network for the memory constraints of a system. Training multiple policies with our method is as sample efficient as training a single policy. Finally, we provide a method to select the best architecture, given a constraint on the number of parameters. Project website: https://sites.google.com/usc.edu/graphhyperpolicy

==> 5_Discussion.tex <==


\section{Discussion}
\label{sec:disc}


\subsection{Other Possible Solutions}
In this subsection we discuss other state of the art approaches that can be re-purposed to achieve smaller control networks.

\begin{figure}[ht]
    \centering
    \includegraphics[width=0.75\columnwidth]{figs/critical_states.png}
  \vspace{0.2cm}
\caption{Policies with higher representational capacity can better approximate the optimal policy, therefore letting it navigate through dense critical states.}
\label{fig:size_matters}
\end{figure}

To theoretically explain the dependency of architecture on performance, we would like to reintroduce the concept of critical states \cite{kumar2022prefer}. 
These states correspond to regions where it is absolutely necessary to take precise optimal actions to complete a task and usually, trajectories with higher reward tend to have a higher concentration of critical states.
While a global optimal policy might navigate through critical states easily, approximations of this policy might not do so. 
In Deep Reinforcement Learning, it common practice to model control policies with functional approximators. 
Therefore naturally the representational capacity of the approximator used will directly impact the strategy learnt with reinforcement learning. With large networks, this is not an issue as the representational capacity of these networks are vast, regardless of the size. But as we reduce the size of the networks, this capacity measure plays a crucial role in determining it's performance.

As shown in Fig \ref{fig:size_matters}, if we model a policy with a network of higher representational capacity, we can effectively navigate through dense critical states. Modeling a policy with a lower representational capacity may learn a strategy that navigates through fewer critical states. 


We can achieve a smaller network to solve a task, using multiple methods. 
\subsubsection{Imitation Learning}
We can train an expert policy with a large number of parameters first. Then we can train a smaller network to imitate this network.
The simplest form of imitation learning is Behaviour cloning \cite{DBLP:journals/corr/abs-2004-00981}. Given a stochastic expert policy $\pi _{E}$, we aim to train a new policy $\pi$ by optimizing the following objective function:
\begin{equation}
\label{eq:bc_obj}
    J_{BC}(\pi , \pi _{E}) = -E_{(a,s)\in \beta_{E}}[log \pi (a | s)] 
\end{equation}
An important fact here, is that the state and action data is sampled from the expert's trajectories $\beta_E$. 
The states observed by the student policy $\pi$ might not follow this distribution, leading to "brittle" performance. 
It was shown by \cite{kumar2022prefer}, that the presence of critical states in the environment leads to poor performance of behaviour cloning. 
The exact same argument can be made for distilling knowledge into smaller networks. 
As shown in Fig \ref{fig:size_matters}, a larger network may not visit trajectories with lesser critical states, therefore cause the state distribution shift problem. This explains the sub par performance of behaviour cloning in Table \ref{tab:perf}

\subsubsection{Model Pruning}
We can first train an expert policy $\pi _{E}$ and then reduce the size of this network by removing some of its parameters. 
This removal can be done while minimizing its impact on the output of the network. 
For image classification, multiple methods of pruning have been shown to reduce the network size by upto 50\% while reducing its accuracy to 50\% \cite{DBLP:journals/corr/abs-2003-03033}.  
But we argue that this might not be the case for models trained on regression tasks, which account for most of robotic control policies. 
Further, small errors in output can compound over time causing a reduction in performance. 

A promising approach was suggested by \cite{DBLP:journals/corr/abs-1803-03635}, to perform magnitude pruning in an iterated fashion. 
This was originally introduced for image classification.
Later, \cite{DBLP:journals/corr/abs-2105-01648} performed this method for reinforcement learning, and showed how we can achieve much smaller control network by distilling knowledge from a larger teacher to a smaller student using iterated magnitude pruning (IMP). 
But, for the locomotion tasks that we have benchmarked our method on, the best performance they could achieve was much lower.
This is primarily because their method was based on behavioural cloning, which even when used to distil knowledge to a similarly scaled network, would achieve lower performance. 

\subsubsection{Offline Reinforcement Learning}
Another way to distill knowledge from one network to another is by using Offline reinforcement learning \cite{DBLP:journals/corr/abs-2005-01643} on data collected from an expert model. 
This is a field that has garnered a lot of attention recently. 
Using the data collected remotely from any source, we can train a control policy that optimizes on this data.
But as was initially pointed out by \cite{DBLP:journals/corr/abs-2007-09055}, Offline RL is not robust to hyper parameter selection.
Further, state of the art results using offline RL to distill knowledge into a network, generally achieves performance much lower than the expert \cite{DBLP:journals/corr/abs-2004-07219}. All this makes training high performing smaller networks much harder.

\subsection{Limitations}
We would finally like to point out a few limitations in our method. The GHN used to model a graph hyper policy is large. 
While our objective is to achieve smaller MLP's during execution time, the size of the actor network is much larger during training, increasing the training time significantly. 
Since this is an engineering issue, the implementation of the Off Policy algorithm used is critical in reducing training time 
With our single GPU implementations, even though the samples complexity did not increase, the total training time saw an increase of 4-5 times. 

